An Experiment in Retrofitting Competency Questions for Existing Ontologies

Competency Questions (CQs) are a form of ontology functional requirements expressed as natural language questions. Inspecting CQs together with the axioms in an ontology provides critical insights into the intended scope and applicability of the ontology. CQs also underpin a number of tasks in the development of ontologies e.g. ontology reuse, ontology testing, requirement specification, and the definition of patterns that implement such requirements. Although CQs are integral to the majority of ontology engineering methodologies, the practice of publishing CQs alongside the ontological artefacts is not widely observed by the community. In this context, we present an experiment in retrofitting CQs from existing ontologies. We propose RETROFIT-CQs, a method to extract candidate CQs directly from ontologies using Generative AI. In the paper we present the pipeline that facilitates the extraction of CQs by leveraging Large Language Models (LLMs) and we discuss its application to a number of existing ontologies.

==> refrences/KCAP2023_complete.tex <==
%NEW KCAP 2023 BIB
@InProceedings{Oscar2022,
author="Espinoza-Arias, Paola
and Garijo, Daniel
and Corcho, Oscar",
editor1="Corcho, Oscar
and Hollink, Laura
and Kutz, Oliver
and Troquard, Nicolas
and Ekaputra, Fajar J.",
title="Extending Ontology Engineering Practices to Facilitate Application Development",
booktitle="Knowledge Engineering and Knowledge Management",
year="2022",
publisher="Springer International Publishing",
address1 ="Cham, Switzerland"
pages="19--35"
}
%CEhck how to cite this workshop paper 

@article{mynarz2023test,
  title={Test-driven knowledge graph construction},
  author={Mynarz, Jind{\v{r}}ich and Hanikov{\'a}, Kate{\v{r}}ina and Sv{\'a}tek, Vojt{\v{e}}ch},
  year={2023}
}

@article{Jorege2023,
title = {KNIT: Ontology reusability through knowledge graph exploration},
journal = {Expert Systems with Applications},
volume = {228},
pages = {120239},
year = {2023},
author = {Jorge Rodríguez-Revello and Cristóbal Barba-González and Maciej Rybinski and Ismael Navas-Delgado},
doi ={10.1016/j.eswa.2023.120239}
}

@Incollection{gruninger1995methodology,
author="Gr{\"u}ninger, Michael
and Fox, Mark S.",
editor1="Rolstad{\aa}s, Asbj{\o}rn",
title="The Role of Competency Questions in Enterprise Engineering",
bookTitle="Benchmarking --- Theory and Practice",
year="1995",
publisher="Springer US",
address1="Boston, MA",
pages="22--31",
abstract="We present a logical framework for representing activities, states, time, and cost in an enterprise integration architecture. We define ontologies for these concepts in first-order logic and consider the problems of temporal projection and reasoning about the occurrence of actions. We characterize the ontology with the use of competency questions. The ontology must contain a necessary and sufficient set of axioms to represent and solve these questions. These questions not only characterize existing ontologies for enterprise engineering, but also drive the development of new ontologies that are required to solve the competency questions.",
isbn1="978-0-387-34847-6",
doi1="10.1007/978-0-387-34847-6_3",
url1="https://doi.org/10.1007/978-0-387-34847-6_3"
}

@inproceedings{DBLP:conf/i-semantics/GangemiLLN22,
  author       = {Aldo Gangemi and
                  Anna Sofia Lippolis and
                  Giorgia Lodi and
                  Andrea Giovanni Nuzzolese},
  editor1       = {Anastasia Dimou and
                  Sebastian Neumaier and
                  Tassilo Pellegrini and
                  Sahar Vahdati},
  title        = {Automatically Drafting Ontologies from Competency Questions with FrODO},
  booktitle    = {Towards a Knowledge-Aware {AI} - SEMANTiCS 2022 - Proceedings of the
                  18th International Conference on Semantic Systems, 13-15 September
                  2022, Vienna, Austria},
  series       = {Studies on the Semantic Web},
  volume       = {55},
  pages        = {107--121},
  publisher    = {{IOS} Press},
  year         = {2022},
  url1          = {https://doi.org/10.3233/SSW220014},
  doi1          = {10.3233/SSW220014},
  timestamp1    = {Mon, 17 Oct 2022 08:33:06 +0200},
  biburl1       = {https://dblp.org/rec/conf/i-semantics/GangemiLLN22.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}
a service of  Schloss Dagstuhl - Leibniz Center for Informatics	homebrowsesearchaboutnfdi


@InProceedings{coral,
author="Fern{\'a}ndez-Izquierdo, Alba
and Poveda-Villal{\'o}n, Mar{\'i}a
and Garc{\'i}a-Castro, Ra{\'u}l",
editor1="Hitzler, Pascal
and Fern{\'a}ndez, Miriam
and Janowicz, Krzysztof
and Zaveri, Amrapali
and Gray, Alasdair J.G.
and Lopez, Vanessa
and Haller, Armin
and Hammar, Karl",
title="CORAL: A Corpus of Ontological Requirements Annotated with Lexico-Syntactic Patterns",
booktitle="The Semantic Web, 16th International Conference, ESWC 2019",
address1= "Cham, Switzerland",
year="2019",
publisher="Springer International Publishing",
pages="443--458"}

@article{wisniewski2019analysis,
  title={Analysis of Ontology Competency Questions and their formalizations in SPARQL-OWL},
  author={Wi{\'s}niewski, Dawid and Potoniec, Jedrzej and {\L}awrynowicz, Agnieszka and Keet, C Maria},
  journal={Journal of Web Semantics},
  volume={59},
  pages={100534},
  year={2019},
  publisher={Elsevier},
  doi1 = {10.1016/j.websem.2019.100534}
}


@article{POTONIEC2020105098,
title = {Dataset of ontology competency questions to SPARQL-OWL queries translations},
journal = {Data in Brief},
volume = {29},
pages = {105098},
year = {2020},
issn1 = {2352-3409},
doi1 = {https://doi.org/10.1016/j.dib.2019.105098},
url1 = {https://www.sciencedirect.com/science/article/pii/S2352340919314544},
author = {Jedrzej Potoniec and Dawid Wiśniewski and Agnieszka Ławrynowicz and C. Maria Keet},
keywords = {Ontology authoring, Competency questions, SPARQL-OWL, Semantic web},
abstract = {This data article reports on a new set of 234 competency questions for ontology development and their formalisation into a set of 131 SPARQL-OWL queries. This is the largest set of competency questions with their linked queries to date, covering several ontologies of different type in different subject domains developed by different groups of question authors and ontology developers. The dataset is focused specifically on the ontology TBox (terminological part). The dataset may serve as a manually created gold standard for testing and benchmarking, research into competency questions and querying ontologies, and tool development. The data is available in Mendeley Data. Its analysis is presented in “Analysis of Ontology Competency Questions and their formalizations in SPARQL-OWL” [15].}
}

@article{adee4fe404784a1a955f5d15beb11e81,
title = "MIRO: Guidelines for Minimum Information for the Reporting of an Ontology",
keywords = "Ontologies, reporting guidelines, minimum information, ontology reporting",
author = "Nicolas Matentzoglu and James Malone and Chris Mungall and Robert Stevens",
year = "2018",
doi1 = "10.1186/s13326-017-0172-7",
language1 = "English",
journal = "Biomedical Semantics",
issn1 = "2041-1480",
publisher = "Springer Nature",

}

@inproceedings{Alharbi2021AssessingCO,
  title={Assessing Candidate Ontologies for Reuse},
  author={Reham Alharbi},
  booktitle={Proceedings of the Doctoral Consortium at ISWC 2021 (ISWC-DC)},
  year={2021},
  url1={https://api.semanticscholar.org/CorpusID:244895203}
}


@InProceedings{juan2019,
author="Sequeda, Juan F.
and Briggs, Willard J.
and Miranker, Daniel P.
and Heideman, Wayne P.",
editor1="Ghidini, Chiara
and Hartig, Olaf
and Maleshkova, Maria
and Sv{\'a}tek, Vojt{\v{e}}ch
and Cruz, Isabel
and Hogan, Aidan
and Song, Jie
and Lefran{\c{c}}ois, Maxime
and Gandon, Fabien",
title="A Pay-as-you-go Methodology to Design and Build Enterprise Knowledge Graphs from Relational Databases",
booktitle="The Semantic Web -- ISWC 2019",
year="2019",
publisher="Springer International Publishing",
pages="526--545",
doi1= {10.1007/978-3-030-30796-7_32}
}

@article{SurezFigueroa2015NEON,
  title={The NeOn Methodology framework: A scenario-based methodology for ontology development},
  author={Mari Carmen Su{\'a}rez-Figueroa and Asunci{\'o}n G{\'o}mez-P{\'e}rez and Mariano Fern{\'a}ndez-L{\'o}pez},
  journal={Applied ontology},
  volume = {10},
  number = {2},
  year={2015},
  publisher={IOS Press},
  pages={107-145}
}


@inproceedings{Presutti2009eXtremeDW,
author = {Presutti, Valentina and Daga, Enrico and Gangemi, Aldo and Blomqvist, Eva},
title = {EXtreme Design with Content Ontology Design Patterns},
year = {2009},
publisher = {CEUR-WS.org},
booktitle = {Proceedings of the 2009 International Conference on Ontology Patterns},
pages = {83–97},
series = {WOP'09}}

@misc{noy2001ontology,
  title={Ontology development 101: A guide to creating your first ontology},
  author={Noy, Natalya F and McGuinness, Deborah L and others},
  year={2001},
  publisher={Stanford knowledge systems laboratory technical report KSL-01-05 and~…}
}

@article{Staab2001,
author = {Staab, Steffen and Studer, Rudi and Schnurr, Hans-Peter and Sure, York},
title = {Knowledge Processes and Ontologies},
year = {2001},
publisher = {IEEE Educational Activities Department},
volume = {16},
number = {1},
doi1 = {10.1109/5254.912382},
journal = {IEEE Intelligent Systems},
pages = {26–34}
}

@inproceedings{Bezerra2017,
  author       = {Camila Bezerra and
                  Fred Freitas},
  editor1       = {Mara Abel and
                  Sandro Rama Fiorini and
                  Christiano Pessanha},
  title        = {Verifying Description Logic Ontologies based on Competency Questions
                  and Unit Testing},
  booktitle    = {Proceedings of the {IX} Seminar on Ontology Research in Brazil and
                  {I} Doctoral and Masters Consortium on Ontologies, Bras{\'{\i}}lia,
                  Brazil, August 28th-30th, 2017},
  series       = {{CEUR} Workshop Proceedings},
  volume       = {1908},
  pages        = {159--164},
  publisher    = {CEUR-WS.org},
  address1      = {Aachen, Germany},
  year         = {2017},
  url1          = {https://ceur-ws.org/Vol-1908/paper16.pdf},
  timestamp1    = {Fri, 10 Mar 2023 16:22:15 +0100},
  biburl1       = {https://dblp.org/rec/conf/ontobras/BezerraF17.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pai/MullaG23,
  author       = {Nikahat Mulla and
                  Prachi Gharpure},
  title        = {Automatic question generation: a review of methodologies, datasets,
                  evaluation metrics, and applications},
  journal      = {Prog. Artif. Intell.},
  volume       = {12},
  number       = {1},
  pages        = {1--32},
  year         = {2023},
  url1          = {https://doi.org/10.1007/s13748-023-00295-9},
  doi1          = {10.1007/s13748-023-00295-9},
  timestamp1    = {Sun, 16 Apr 2023 20:30:57 +0200},
  biburl1       = {https://dblp.org/rec/journals/pai/MullaG23.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/Ouyang0JAWMZASR22,
  author       = {Long Ouyang and
                  Jeffrey Wu and
                  Xu Jiang and
                  Diogo Almeida and
                  Carroll L. Wainwright and
                  Pamela Mishkin and
                  Chong Zhang and
                  Sandhini Agarwal and
                  Katarina Slama and
                  Alex Ray and
                  John Schulman and
                  Jacob Hilton and
                  Fraser Kelton and
                  Luke Miller and
                  Maddie Simens and
                  Amanda Askell and
                  Peter Welinder and
                  Paul F. Christiano and
                  Jan Leike and
                  Ryan Lowe},
  title        = {Training language models to follow instructions with human feedback},
  booktitle    = {NeurIPS},
  year         = {2022},
  url1          = {http://papers.nips.cc/paper\_files/paper/2022/hash/b1efde53be364a73914f58805a001731-Abstract-Conference.html},
  timestamp1    = {Thu, 11 May 2023 17:08:21 +0200},
  biburl1       = {https://dblp.org/rec/conf/nips/Ouyang0JAWMZASR22.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/csur/LiuYFJHN23,
  author       = {Pengfei Liu and
                  Weizhe Yuan and
                  Jinlan Fu and
                  Zhengbao Jiang and
                  Hiroaki Hayashi and
                  Graham Neubig},
  title        = {Pre-train, Prompt, and Predict: {A} Systematic Survey of Prompting
                  Methods in Natural Language Processing},
  journal      = {{ACM} Comput. Surv.},
  volume       = {55},
  number       = {9},
  pages        = {195:1--195:35},
  year         = {2023},
  url1          = {https://doi.org/10.1145/3560815},
  doi1          = {10.1145/3560815},
  timestamp1    = {Mon, 28 Aug 2023 21:19:32 +0200},
  biburl1       = {https://dblp.org/rec/journals/csur/LiuYFJHN23.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2201-05337,
  author       = {Hanqing Zhang and
                  Haolin Song and
                  Shaoyu Li and
                  Ming Zhou and
                  Dawei Song},
  title        = {A Survey of Controllable Text Generation using Transformer-based Pre-trained
                  Language Models},
  journal      = {CoRR},
  volume       = {abs/2201.05337},
  year         = {2022},
  url1          = {https://arxiv.org/abs/2201.05337},
  eprinttype1    = {arXiv},
  eprint1       = {2201.05337},
  timestamp1    = {Mon, 30 Jan 2023 17:37:17 +0100},
  biburl1       = {https://dblp.org/rec/journals/corr/abs-2201-05337.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Dennis2017,
author="Dennis, Matt
and van Deemter, Kees
and Dell'Aglio, Daniele
and Pan, Jeff Z.",
editor1="d'Amato, Claudia
and Fernandez, Miriam
and Tamma, Valentina
and Lecue, Freddy
and Cudr{\'e}-Mauroux, Philippe
and Sequeda, Juan
and Lange, Christoph
and Heflin, Jeff",
title="Computing Authoring Tests from Competency Questions: Experimental Validation",
booktitle="The Semantic Web -- ISWC 2017",
year="2017",
publisher="Springer International Publishing",
pages="243--259",
doi1={10.1007/978-3-319-68288-4_15}
}

@InProceedings{Ren2014,
author="Ren, Yuan
and Parvizi, Artemis
and Mellish, Chris
and Pan, Jeff Z.
and van Deemter, Kees
and Stevens, Robert",
editor1="Presutti, Valentina
and d'Amato, Claudia
and Gandon, Fabien
and d'Aquin, Mathieu
and Staab, Steffen
and Tordai, Anna",
title="Towards Competency Question-Driven Ontology Authoring",
booktitle="The Semantic Web: Trends and Challenges",
year="2014",
publisher="Springer International Publishing",
pages="752--767",
doi1={10.1007/978-3-319-07443-6_50}
}

@InProceedings{SurezFigueroa2009,
author="Su{\'a}rez-Figueroa, Mari Carmen
and G{\'o}mez-P{\'e}rez, Asunci{\'o}n
and Villaz{\'o}n-Terrazas, Boris",
editor1="Meersman, Robert
and Dillon, Tharam
and Herrero, Pilar",
title="How to Write and Use the Ontology Requirements Specification Document",
booktitle="On the Move to Meaningful Internet Systems: OTM 2009",
year="2009",
publisher="Springer Berlin Heidelberg",
pages="966--982",
doi1={10.1007/978-3-642-05151-7_16}
}

@inproceedings{Ghomari2013TranslatingNL,
  title={Translating Natural Language Competency Questions into SPARQLQueries: A Case Study},
  author={Leila Zemmouchi-Ghomari and Abdessamed R{\'e}da Ghomari},
  booktitle={The First International Conference on Building and Exploring Web Based Environments},
  pages="81--86",
  year={2013}
}

@InProceedings{CLARO2019,
author="Keet, C. Maria
and Mahlaza, Zola
and Antia, Mary-Jane",
editor1="Garoufallou, Emmanouel
and Fallucchi, Francesca
and William De Luca, Ernesto",
title="CLaRO: A Controlled Language for Authoring Competency Questions",
booktitle="Metadata and Semantic Research",
year="2019",
publisher="Springer International Publishing",
address1 = "Cham, Switzerland"
pages="3--15",
doi1={10.1007/978-3-030-36599-8_1}
}

@article{Bezerra2014CQCheckerAT,
  title={CQChecker: A Tool to Check Ontologies in OWL-DL using Competency Questions written in Controlled Natural Language},
  author={Camila Bezerra and Filipe Santana and Frederico Luiz Gonçalves de Freitas},
  journal={Learning and Nonlinear Models},
  year={2014},
  volume={12},
  number={s},
  pages={115-129}
}

@article{jacksonBioPrtal2021,
    author = {Jackson, Rebecca and Matentzoglu, Nicolas and Overton, James A and Vita, Randi and Balhoff, James P and Buttigieg, Pier Luigi and Carbon, Seth and Courtot, Melanie and Diehl, Alexander D and Dooley, Damion M and Duncan, William D and Harris, Nomi L and Haendel, Melissa A and Lewis, Suzanna E and Natale, Darren A and Osumi-Sutherland, David and Ruttenberg, Alan and Schriml, Lynn M and Smith, Barry and Stoeckert Jr., Christian J and Vasilevsky, Nicole A and Walls, Ramona L and Zheng, Jie and Mungall, Christopher J and Peters, Bjoern},
    title = "{OBO Foundry in 2021: operationalizing open data principles to evaluate ontologies}",
    journal = {Database},
    volume = {2021},
    doi1 = {10.1093/database/baab069}
}


@misc{gozalobrizuela2023chatgpt,
      title={ChatGPT is not all you need. A State of the Art Review of large Generative AI models}, 
      author={Roberto Gozalo-Brizuela and Eduardo C. Garrido-Merchan},
      year={2023},
      eprint={2301.04655},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      doi1={10.48550/arXiv.2301.04655}
}

@article{zhai2022chatgpt,
  title={ChatGPT user experience: Implications for education},
  author={Zhai, Xiaoming},
  journal={Available at SSRN 4312418},
  year={2022},
doi1={10.2139/ssrn.4312418}
}

@misc{barke2022grounded,
      title={Grounded Copilot: How Programmers Interact with Code-Generating Models}, 
      author={Shraddha Barke and Michael B. James and Nadia Polikarpova},
      year={2022},
      eprint={2206.15000},
      archivePrefix={arXiv},
      primaryClass={cs.HC},
doi1={10.48550/arXiv.2206.15000}
}

@inproceedings{Priyan2022codeG,
author = {Vaithilingam, Priyan and Zhang, Tianyi and Glassman, Elena L.},
title = {Expectation vs. Experience: Evaluating the Usability of Code Generation Tools Powered by Large Language Models},
year = {2022},
isbn1 = {9781450391566},
publisher = {Association for Computing Machinery},
doi1 = {10.1145/3491101.3519665},
booktitle = {Extended Abstracts of the 2022 CHI Conference on Human Factors in Computing Systems},
series = {CHI EA '22}
}

@article{Nigar2023, 
title={Use Chat GPT to Solve Programming Bugs},
volume={3}, 
DOI1={10.55529/ijitc.31.17.22},
number={01}, 
journal={International Journal of Information Technology and Computer Engineering (IJITC) ISSN : 2455-5290}, 
author={Nigar M. Shafiq Surameery and Mohammed Y. Shakor}, 
year={2023}, 
pages={17–22} }

@misc{openai2021chatgpt,
  author = {OpenAI},
  title = {ChatGPT: Language Models for Conversational AI, Available online:},
  year = {accessed on 16 July 2023},
  url = {https://beta.openai.com/docs/models}
}


@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}

@article{POVEDAVILLALON2022LOT,
title = {LOT: An industrial oriented ontology engineering framework},
journal = {Engineering Applications of Artificial Intelligence},
volume = {111},
pages = {104755},
year = {2022},
author = {María Poveda-Villalón and Alba Fernández-Izquierdo and Mariano Fernández-López and Raúl García-Castro},
doi1 = {10.1016/j.engappai.2022.104755}}

@InProceedings{Keettestdriven2016,
author="Keet, C. Maria
and {\L}awrynowicz, Agnieszka",
editor1="Sack, Harald
and Blomqvist, Eva
and d'Aquin, Mathieu
and Ghidini, Chiara
and Ponzetto, Simone Paolo
and Lange, Christoph",
title="Test-Driven Development of Ontologies",
booktitle="The Semantic Web. Latest Advances and New Domains",
year="2016",
publisher="Springer International Publishing",
address1 = "Cham, Switzerland",
pages="642--657",
doi1={10.1007/978-3-319-34129-3_39}
}

@article{KeetDataset2020,
title = {Dataset of ontology competency questions to SPARQL-OWL queries translations},
journal = {Data in Brief},
volume = {29},
pages = {105098},
year = {2020},
issn1 = {2352-3409},
doi1 = {10.1016/j.dib.2019.105098},
author = {Jedrzej Potoniec and Dawid Wiśniewski and Agnieszka Ławrynowicz and C. Maria Keet}
}


@inproceedings{Bezerra2017duplicatetoremove,
  author       = {Camila Bezerra and
                  Fred Freitas},
  editor1       = {Mara Abel and
                  Sandro Rama Fiorini and
                  Christiano Pessanha},
  title        = {Verifying Description Logic Ontologies based on Competency Questions
                  and Unit Testing},
  booktitle    = {Proceedings of the {IX} Seminar on Ontology Research in Brazil and
                  {I} Doctoral and Masters Consortium on Ontologies, Bras{\'{\i}}lia,
                  Brazil, August 28th-30th, 2017},
  series       = {{CEUR} Workshop Proceedings},
  volume       = {1908},
  pages        = {159--164},
  publisher    = {CEUR-WS.org},
  year         = {2017}
}

@article{Deng_Lin_2023, 
title={The Benefits and Challenges of ChatGPT: An Overview},
volume={2}, 
DOI1={10.54097/fcis.v2i2.4465}, 
number={2}, 
journal={Frontiers in Computing and Intelligent Systems}, 
author={Deng, Jianyang and Lin, Yijia}, 
year={2023}, 
pages={81–83} }

@ARTICLE{Dave2023,
  title    = "{ChatGPT} in medicine: an overview of its applications,
              advantages, limitations, future prospects, and ethical
              considerations",
  author   = "Dave, Tirth and Athaluri, Sai Anirudh and Singh, Satyam",
  journal  = "Front Artif Intell",
  volume   =  "6",
  pages    = "1169595",
  year     =  "2023",
  
}

@INPROCEEDINGS{Qadir2023,
  author={Qadir, Junaid},
  booktitle={2023 IEEE Global Engineering Education Conference (EDUCON)}, 
  title={Engineering Education in the Era of ChatGPT: Promise and Pitfalls of Generative AI for Education}, 
  year={2023},
  volume={},
  number={},
  pages={1-9},
  doi1={10.1109/EDUCON54358.2023.10125121}}

@inproceedings{reimers-gurevych-2019-sentence,
    title = "Sentence-{BERT}: Sentence Embeddings using {S}iamese {BERT}-Networks",
    author = "Reimers, Nils  and
      Gurevych, Iryna",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    year = "2019",
    publisher = "Association for Computational Linguistics",
    doi1 = "10.18653/v1/D19-1410",
    pages = "3982--3992"   
}

@article{Parkkila2017AnOF,
  title={An ontology for videogame interoperability},
  author={Janne Parkkila and Filip Radulovic and Daniel Garijo and Mar{\'i}a Poveda-Villal{\'o}n and Jouni Ikonen and Jari Porras and Asunci{\'o}n G{\'o}mez-P{\'e}rez},
  journal={Multimedia Tools and Applications},
  year={2017},
  volume={76},
  pages={4981-5000}
}

@techreport{smartm2m,
    title = {SmartM2M: SAREF Extension Investigation},
    type = {Technical Report},
    number = {TR 103 411},
    year={2017}
}

@book{montiel2011multilingualism,
  title={Multilingualism in Ontologies - Building Patterns and Representation Models},
  author={Montiel-Ponsoda, E.},
  publisher={LAP Lambert Academic Publishing},
  address1={Germany},
  year={2011}
}

@InProceedings{Aziz2023,
author="Azzi, Sabrina
and Assi, Ali
and Gagnon, St{\'e}phane",
editor1="Garoufallou, Emmanouel
and Vlachidis, Andreas",
title="Scoring Ontologies for Reuse: An Approach for Fitting Semantic Requirements",
booktitle="Metadata and Semantic Research",
year="2023",
publisher="Springer Nature",
address1 = "Cham, Switzerland",
pages="203--208",
doi1={10.1007/978-3-031-39141-5_17}
}

@inproceedings{alharbiKcap2021,
author = {Alharbi, Reham and Tamma, Valentina and Grasso, Floriana},
title = {Characterising the Gap Between Theory and Practice of Ontology Reuse},
year = {2021},
publisher = {Association for Computing Machinery},
doi1 = {10.1145/3460210.3493568},
booktitle = {Proceedings of the 11th on Knowledge Capture Conference},
pages = {217–224},
numpages = {8},
series = {K-CAP '21}
}

@article{GangemiEtAl2017,
  author = {Gangemi, Aldo and Presutti, Valentina and Recupero, Diego Reforgiato and Nuzzolese, Andrea Giovanni and Draicchio, Francesco and MongiovÃ¬, Misael},
  journal = {Semantic Web},
  number = 6,
  pages = {873-893},
  title = {{Semantic Web Machine Reading with FRED}},
  volume = 8,
  year = 2017
}

@inproceedings{DBLP:conf/acl/ImaniD023,
  author       = {Shima Imani and
                  Liang Du and
                  Harsh Shrivastava},
  title        = {MathPrompter: Mathematical Reasoning using Large Language Models},
  booktitle    = {Proceedings of the The 61st Annual Meeting of the Association for
                  Computational Linguistics: Industry Track, {ACL} 2023, Toronto, Canada,
                  July 9-14, 2023},
  pages        = {37--42},
  year         = {2023},
}

@inproceedings{AlkhuzaeyECEL23,
  title={A Framework for Assessing the Complexity of Auto Generated Questions from Ontologies},
  author={Samah AlKhuzaey and Floriana Grasso and Terry R. Payne and Valentina Tamma},
  booktitle={Proc. of the 22nd European Conf. on e-Learning (to appear)},
  year={2023}
}
@book{10.1145/3382097, 
author = {Allemang, Dean and Hendler, Jim and Gandon, Fabien}, title = {Semantic Web for the Working Ontologist: Effective Modeling for Linked Data, RDFS, and OWL}, year = {2020}, isbn = {9781450376174}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, edition = {3}, volume = {33}, abstract = {Enterprises have made amazing advances by taking advantage of data about their business to provide predictions and understanding of their customers, markets, and products. But as the world of business becomes more interconnected and global, enterprise data is no long a monolith; it is just a part of a vast web of data. Managing data on a world-wide scale is a key capability for any business today.The Semantic Web treats data as a distributed resource on the scale of the World Wide Web, and incorporates features to address the challenges of massive data distribution as part of its basic design. The aim of the first two editions was to motivate the Semantic Web technology stack from end-to-end; to describe not only what the Semantic Web standards are and how they work, but also what their goals are and why they were designed as they are. It tells a coherent story from beginning to end of how the standards work to manage a world-wide distributed web of knowledge in a meaningful way.The third edition builds on this foundation to bring Semantic Web practice to enterprise. Fabien Gandon joins Dean Allemang and Jim Hendler, bringing with him years of experience in global linked data, to open up the story to a modern view of global linked data. While the overall story is the same, the examples have been brought up to date and applied in a modern setting, where enterprise and global data come together as a living, linked network of data. Also included with the third edition, all of the data sets and queries are available online for study and experimentation at data.world/swwo.} }


%%%%% THE END OF KCAP 2023 BIB %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%% THE END OF KCAP 2023 BIB %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> refrences/Kcap_completed.tex <==
%NEW KCAP 2023 BIB
@InProceedings{Oscar2022,
author="Espinoza-Arias, Paola
and Garijo, Daniel
and Corcho, Oscar",
editor1="Corcho, Oscar
and Hollink, Laura
and Kutz, Oliver
and Troquard, Nicolas
and Ekaputra, Fajar J.",
title="Extending Ontology Engineering Practices to Facilitate Application Development",
booktitle="Knowledge Engineering and Knowledge Management",
year="2022",
publisher1="Springer International Publishing",
address1 ="Cham, Switzerland",
pages="19--35"
}
%CEhck how to cite this workshop paper 

@article{mynarz2023test,
  title={Test-driven knowledge graph construction},
  author={Mynarz, Jind{\v{r}}ich and Hanikov{\'a}, Kate{\v{r}}ina and Sv{\'a}tek, Vojt{\v{e}}ch},
  year={2023}
}

@article{Jorege2023,
title = {KNIT: Ontology reusability through knowledge graph exploration},
journal = {Expert Systems with Applications},
volume = {228},
pages = {120239},
year = {2023},
author = {Jorge Rodríguez-Revello and Cristóbal Barba-González and Maciej Rybinski and Ismael Navas-Delgado},
doi ={10.1016/j.eswa.2023.120239}
}

@Incollection{gruninger1995methodology,
author="Gr{\"u}ninger, Michael
and Fox, Mark S.",
editor1="Rolstad{\aa}s, Asbj{\o}rn",
title="The Role of Competency Questions in Enterprise Engineering",
bookTitle="Benchmarking --- Theory and Practice",
year="1995",
publisher="Springer US",
address1="Boston, MA",
pages="22--31",
abstract="We present a logical framework for representing activities, states, time, and cost in an enterprise integration architecture. We define ontologies for these concepts in first-order logic and consider the problems of temporal projection and reasoning about the occurrence of actions. We characterize the ontology with the use of competency questions. The ontology must contain a necessary and sufficient set of axioms to represent and solve these questions. These questions not only characterize existing ontologies for enterprise engineering, but also drive the development of new ontologies that are required to solve the competency questions.",
isbn1="978-0-387-34847-6",
doi1="10.1007/978-0-387-34847-6_3",
url1="https://doi.org/10.1007/978-0-387-34847-6_3"
}

@inproceedings{DBLP:conf/i-semantics/GangemiLLN22,
  author       = {Aldo Gangemi and
                  Anna Sofia Lippolis and
                  Giorgia Lodi and
                  Andrea Giovanni Nuzzolese},
  editor1       = {Anastasia Dimou and
                  Sebastian Neumaier and
                  Tassilo Pellegrini and
                  Sahar Vahdati},
  title        = {Automatically Drafting Ontologies from Competency Questions with FrODO},
  booktitle1    = {Towards a Knowledge-Aware {AI} - SEMANTiCS 2022 - Proceedings of the
                  18th International Conference on Semantic Systems, 13-15 September
                  2022, Vienna, Austria},
booktitle    = {Towards a Knowledge-Aware {AI} - SEMANTiCS 2022 - Proceedings of the
                  18th International Conference on Semantic Systems},
  series       = {Studies on the Semantic Web},
  volume       = {55},
  pages        = {107--121},
  publisher    = {{IOS} Press},
  year         = {2022},
  url1          = {https://doi.org/10.3233/SSW220014},
  doi1          = {10.3233/SSW220014},
  timestamp1    = {Mon, 17 Oct 2022 08:33:06 +0200},
  biburl1       = {https://dblp.org/rec/conf/i-semantics/GangemiLLN22.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}
a service of  Schloss Dagstuhl - Leibniz Center for Informatics	homebrowsesearchaboutnfdi


@InProceedings{coral,
author="Fern{\'a}ndez-Izquierdo, Alba
and Poveda-Villal{\'o}n, Mar{\'i}a
and Garc{\'i}a-Castro, Ra{\'u}l",
editor1="Hitzler, Pascal
and Fern{\'a}ndez, Miriam
and Janowicz, Krzysztof
and Zaveri, Amrapali
and Gray, Alasdair J.G.
and Lopez, Vanessa
and Haller, Armin
and Hammar, Karl",
title="CORAL: A Corpus of Ontological Requirements Annotated with Lexico-Syntactic Patterns",
booktitle="The Semantic Web, 16th International Conference, ESWC 2019",
address1= "Cham, Switzerland",
year="2019",
publisher="Springer International Publishing",
pages="443--458"}

@article{wisniewski2019analysis,
  title={Analysis of Ontology Competency Questions and their formalizations in SPARQL-OWL},
  author={Wi{\'s}niewski, Dawid and Potoniec, Jedrzej and {\L}awrynowicz, Agnieszka and Keet, C Maria},
  journal={Journal of Web Semantics},
  volume={59},
  pages={100534},
  year={2019},
  publisher={Elsevier}
}


@article{POTONIEC2020105098,
title = {Dataset of ontology competency questions to SPARQL-OWL queries translations},
journal = {Data in Brief},
volume = {29},
pages = {105098},
year = {2020},
issn1 = {2352-3409},
doi1 = {https://doi.org/10.1016/j.dib.2019.105098},
url1 = {https://www.sciencedirect.com/science/article/pii/S2352340919314544},
author = {Jedrzej Potoniec and Dawid Wiśniewski and Agnieszka Ławrynowicz and C. Maria Keet},
keywords = {Ontology authoring, Competency questions, SPARQL-OWL, Semantic web},
abstract = {This data article reports on a new set of 234 competency questions for ontology development and their formalisation into a set of 131 SPARQL-OWL queries. This is the largest set of competency questions with their linked queries to date, covering several ontologies of different type in different subject domains developed by different groups of question authors and ontology developers. The dataset is focused specifically on the ontology TBox (terminological part). The dataset may serve as a manually created gold standard for testing and benchmarking, research into competency questions and querying ontologies, and tool development. The data is available in Mendeley Data. Its analysis is presented in “Analysis of Ontology Competency Questions and their formalizations in SPARQL-OWL” [15].}
}

@article{adee4fe404784a1a955f5d15beb11e81,
title = "MIRO: Guidelines for Minimum Information for the Reporting of an Ontology",
keywords = "Ontologies, reporting guidelines, minimum information, ontology reporting",
author = "Nicolas Matentzoglu and James Malone and Chris Mungall and Robert Stevens",
year = "2018",
doi1 = "10.1186/s13326-017-0172-7",
language1 = "English",
journal = "Biomedical Semantics",
issn1 = "2041-1480",
publisher = "Springer Nature",

}

@inproceedings{Alharbi2021AssessingCO,
  title={Assessing Candidate Ontologies for Reuse},
  author={Reham Alharbi},
  booktitle={Proceedings of the Doctoral Consortium at ISWC 2021 (ISWC-DC)},
  year={2021},
  url={https://api.semanticscholar.org/CorpusID:244895203}
}


@InProceedings{juan2019,
author="Sequeda, Juan F.
and Briggs, Willard J.
and Miranker, Daniel P.
and Heideman, Wayne P.",
editor1="Ghidini, Chiara
and Hartig, Olaf
and Maleshkova, Maria
and Sv{\'a}tek, Vojt{\v{e}}ch
and Cruz, Isabel
and Hogan, Aidan
and Song, Jie
and Lefran{\c{c}}ois, Maxime
and Gandon, Fabien",
title="A Pay-as-you-go Methodology to Design and Build Enterprise Knowledge Graphs from Relational Databases",
booktitle="The Semantic Web -- ISWC 2019",
year="2019",
publisher="Springer International Publishing",
pages="526--545",
doi1= {10.1007/978-3-030-30796-7_32}
}

@article{SurezFigueroa2015NEON,
  title={The NeOn Methodology framework: A scenario-based methodology for ontology development},
  author={Mari Carmen Su{\'a}rez-Figueroa and Asunci{\'o}n G{\'o}mez-P{\'e}rez and Mariano Fern{\'a}ndez-L{\'o}pez},
  journal={Applied ontology},
  volume = {10},
  number = {2},
  year={2015},
  publisher={IOS Press},
  pages={107-145}
}


@inproceedings{Presutti2009eXtremeDW,
author = {Presutti, Valentina and Daga, Enrico and Gangemi, Aldo and Blomqvist, Eva},
title = {EXtreme Design with Content Ontology Design Patterns},
year = {2009},
publisher = {CEUR-WS.org},
booktitle = {Proceedings of the 2009 International Conference on Ontology Patterns},
pages = {83–97},
series = {WOP'09}}

@techreport{noy2001ontology,
  title={Ontology development 101: A guide to creating your first ontology},
  author={Noy, Natalya F and McGuinness, Deborah L},
  year={2001},
  publisher={Stanford knowledge systems laboratory technical report KSL-01-05 and~…}
}

@article{Staab2001,
author = {Staab, Steffen and Studer, Rudi and Schnurr, Hans-Peter and Sure, York},
title = {Knowledge Processes and Ontologies},
year = {2001},
publisher = {IEEE Educational Activities Department},
volume = {16},
number = {1},
doi1 = {10.1109/5254.912382},
journal = {IEEE Intelligent Systems},
pages = {26–34}
}

@inproceedings{Bezerra2017,
  author       = {Camila Bezerra and
                  Fred Freitas},
  editor1       = {Mara Abel and
                  Sandro Rama Fiorini and
                  Christiano Pessanha},
  title        = {Verifying Description Logic Ontologies based on Competency Questions
                  and Unit Testing},
booktitle1    = {Proceedings of the {IX} Seminar on Ontology Research in Brazil and
                  {I} Doctoral and Masters Consortium on Ontologies, Bras{\'{\i}}lia,
                  Brazil, August 28th-30th, 2017},
booktitle    = {Proceedings of the {IX} Seminar on Ontology Research in Brazil and
                  {I} Doctoral and Masters Consortium on Ontologies},
  series       = {{CEUR} Workshop Proceedings},
  volume       = {1908},
  pages        = {159--164},
  publisher    = {CEUR-WS.org},
  address1      = {Aachen, Germany},
  year         = {2017},
  url1          = {https://ceur-ws.org/Vol-1908/paper16.pdf},
  timestamp1    = {Fri, 10 Mar 2023 16:22:15 +0100},
  biburl1       = {https://dblp.org/rec/conf/ontobras/BezerraF17.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pai/MullaG23,
  author       = {Nikahat Mulla and
                  Prachi Gharpure},
  title        = {Automatic question generation: a review of methodologies, datasets,
                  evaluation metrics, and applications},
  journal      = {Prog. Artif. Intell.},
  volume       = {12},
  number       = {1},
  pages        = {1--32},
  year         = {2023},
  url1          = {https://doi.org/10.1007/s13748-023-00295-9},
  doi1          = {10.1007/s13748-023-00295-9},
  timestamp1    = {Sun, 16 Apr 2023 20:30:57 +0200},
  biburl1       = {https://dblp.org/rec/journals/pai/MullaG23.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/Ouyang0JAWMZASR22,
  author       = {Long Ouyang and
                  Jeffrey Wu and
                  Xu Jiang and
                  Diogo Almeida and
                  Carroll L. Wainwright and
                  Pamela Mishkin and
                  Chong Zhang and
                  Sandhini Agarwal and
                  Katarina Slama and
                  Alex Ray and
                  John Schulman and
                  Jacob Hilton and
                  Fraser Kelton and
                  Luke Miller and
                  Maddie Simens and
                  Amanda Askell and
                  Peter Welinder and
                  Paul F. Christiano and
                  Jan Leike and
                  Ryan Lowe},
  title        = {Training language models to follow instructions with human feedback},
  booktitle    = {NeurIPS},
  year         = {2022},
  url1          = {http://papers.nips.cc/paper\_files/paper/2022/hash/b1efde53be364a73914f58805a001731-Abstract-Conference.html},
  timestamp1    = {Thu, 11 May 2023 17:08:21 +0200},
  biburl1       = {https://dblp.org/rec/conf/nips/Ouyang0JAWMZASR22.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/csur/LiuYFJHN23,
  author       = {Pengfei Liu and
                  Weizhe Yuan and
                  Jinlan Fu and
                  Zhengbao Jiang and
                  Hiroaki Hayashi and
                  Graham Neubig},
  title        = {Pre-train, Prompt, and Predict: {A} Systematic Survey of Prompting
                  Methods in Natural Language Processing},
  journal      = {{ACM} Comput. Surv.},
  volume       = {55},
  number       = {9},
  pages        = {195:1--195:35},
  year         = {2023},
  url1          = {https://doi.org/10.1145/3560815},
  doi1          = {10.1145/3560815},
  timestamp1    = {Mon, 28 Aug 2023 21:19:32 +0200},
  biburl1       = {https://dblp.org/rec/journals/csur/LiuYFJHN23.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2201-05337,
  author       = {Hanqing Zhang and
                  Haolin Song and
                  Shaoyu Li and
                  Ming Zhou and
                  Dawei Song},
  title        = {A Survey of Controllable Text Generation using Transformer-based Pre-trained
                  Language Models},
  journal      = {CoRR},
  volume       = {abs/2201.05337},
  year         = {2022},
  url1          = {https://arxiv.org/abs/2201.05337},
  eprinttype1    = {arXiv},
  eprint1       = {2201.05337},
  timestamp1    = {Mon, 30 Jan 2023 17:37:17 +0100},
  biburl1       = {https://dblp.org/rec/journals/corr/abs-2201-05337.bib},
  bibsource1    = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Dennis2017,
author="Dennis, Matt
and van Deemter, Kees
and Dell'Aglio, Daniele
and Pan, Jeff Z.",
editor1="d'Amato, Claudia
and Fernandez, Miriam
and Tamma, Valentina
and Lecue, Freddy
and Cudr{\'e}-Mauroux, Philippe
and Sequeda, Juan
and Lange, Christoph
and Heflin, Jeff",
title="Computing Authoring Tests from Competency Questions: Experimental Validation",
booktitle="The Semantic Web -- ISWC 2017",
year="2017",
publisher="Springer International Publishing",
pages="243--259",
doi1={10.1007/978-3-319-68288-4_15}
}

@InProceedings{Ren2014,
author="Ren, Yuan
and Parvizi, Artemis
and Mellish, Chris
and Pan, Jeff Z.
and van Deemter, Kees
and Stevens, Robert",
editor1="Presutti, Valentina
and d'Amato, Claudia
and Gandon, Fabien
and d'Aquin, Mathieu
and Staab, Steffen
and Tordai, Anna",
title="Towards Competency Question-Driven Ontology Authoring",
booktitle="The Semantic Web: Trends and Challenges",
year="2014",
publisher="Springer International Publishing",
pages="752--767",
doi1={10.1007/978-3-319-07443-6_50}
}

@InProceedings{SurezFigueroa2009,
author="Su{\'a}rez-Figueroa, Mari Carmen
and G{\'o}mez-P{\'e}rez, Asunci{\'o}n
and Villaz{\'o}n-Terrazas, Boris",
editor1="Meersman, Robert
and Dillon, Tharam
and Herrero, Pilar",
title="How to Write and Use the Ontology Requirements Specification Document",
booktitle="On the Move to Meaningful Internet Systems: OTM 2009",
year="2009",
publisher="Springer Berlin Heidelberg",
pages="966--982",
doi1={10.1007/978-3-642-05151-7_16}
}

@inproceedings{Ghomari2013TranslatingNL,
  title={Translating Natural Language Competency Questions into SPARQLQueries: A Case Study},
  author={Leila Zemmouchi-Ghomari and Abdessamed R{\'e}da Ghomari},
  booktitle={The First International Conference on Building and Exploring Web Based Environments},
  pages="81--86",
  year={2013}
}

@InProceedings{CLARO2019,
author="Keet, C. Maria
and Mahlaza, Zola
and Antia, Mary-Jane",
editor1="Garoufallou, Emmanouel
and Fallucchi, Francesca
and William De Luca, Ernesto",
title="CLaRO: A Controlled Language for Authoring Competency Questions",
booktitle="Metadata and Semantic Research",
year="2019",
publisher="Springer International Publishing",
address1 = "Cham, Switzerland",
pages="3--15",
doi1={10.1007/978-3-030-36599-8_1}
}

@article{Bezerra2014CQCheckerAT,
  title={CQChecker: A Tool to Check Ontologies in OWL-DL using Competency Questions written in Controlled Natural Language},
  author={Camila Bezerra and Filipe Santana and Frederico Luiz Gonçalves de Freitas},
  journal={Learning and Nonlinear Models},
  year={2014},
  volume={12},
  number={s},
  pages={115-129}
}

@article{jacksonBioPrtal2021,
    author = {Jackson, Rebecca and Matentzoglu, Nicolas and Overton, James A and Vita, Randi and Balhoff, James P and Buttigieg, Pier Luigi and Carbon, Seth and Courtot, Melanie and Diehl, Alexander D and Dooley, Damion M and Duncan, William D and Harris, Nomi L and Haendel, Melissa A and Lewis, Suzanna E and Natale, Darren A and Osumi-Sutherland, David and Ruttenberg, Alan and Schriml, Lynn M and Smith, Barry and Stoeckert Jr., Christian J and Vasilevsky, Nicole A and Walls, Ramona L and Zheng, Jie and Mungall, Christopher J and Peters, Bjoern},
    title = "{OBO Foundry in 2021: operationalizing open data principles to evaluate ontologies}",
    journal = {Database},
    volume = {2021},
    doi1 = {10.1093/database/baab069}
}


@misc{gozalobrizuela2023chatgpt,
      title={ChatGPT is not all you need. A State of the Art Review of large Generative AI models}, 
      author={Roberto Gozalo-Brizuela and Eduardo C. Garrido-Merchan},
      year={2023},
      eprint={2301.04655},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      doi1={10.48550/arXiv.2301.04655}
}

@article{zhai2022chatgpt,
  title={ChatGPT user experience: Implications for education},
  author={Zhai, Xiaoming},
  journal={Available at SSRN 4312418},
  year={2022},
doi1={10.2139/ssrn.4312418}
}

@misc{barke2022grounded,
      title={Grounded Copilot: How Programmers Interact with Code-Generating Models}, 
      author={Shraddha Barke and Michael B. James and Nadia Polikarpova},
      year={2022},
      eprint={2206.15000},
      archivePrefix={arXiv},
      primaryClass={cs.HC},
doi1={10.48550/arXiv.2206.15000}
}

@inproceedings{Priyan2022codeG,
author = {Vaithilingam, Priyan and Zhang, Tianyi and Glassman, Elena L.},
title = {Expectation vs. Experience: Evaluating the Usability of Code Generation Tools Powered by Large Language Models},
year = {2022},
isbn1 = {9781450391566},
publisher = {Association for Computing Machinery},
doi1 = {10.1145/3491101.3519665},
booktitle = {Extended Abstracts of the 2022 CHI Conference on Human Factors in Computing Systems},
series = {CHI EA '22}
}

@article{Nigar2023, 
title={Use Chat GPT to Solve Programming Bugs},
volume={3}, 
DOI1={10.55529/ijitc.31.17.22},
number={01}, 
journal={International Journal of Information Technology and Computer Engineering (IJITC) ISSN : 2455-5290}, 
author={Nigar M. Shafiq Surameery and Mohammed Y. Shakor}, 
year={2023}, 
pages={17–22} }

@misc{openai2021chatgpt,
  author = {OpenAI},
  title = {ChatGPT: Language Models for Conversational AI, Available online:},
  year = {accessed on 16 July 2023},
  url = {https://beta.openai.com/docs/models}
}


@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}

@article{POVEDAVILLALON2022LOT,
title = {LOT: An industrial oriented ontology engineering framework},
journal = {Engineering Applications of Artificial Intelligence},
volume = {111},
pages = {104755},
year = {2022},
author = {María Poveda-Villalón and Alba Fernández-Izquierdo and Mariano Fernández-López and Raúl García-Castro},
doi1 = {10.1016/j.engappai.2022.104755}}

@InProceedings{Keettestdriven2016,
author="Keet, C. Maria
and {\L}awrynowicz, Agnieszka",
editor1="Sack, Harald
and Blomqvist, Eva
and d'Aquin, Mathieu
and Ghidini, Chiara
and Ponzetto, Simone Paolo
and Lange, Christoph",
title="Test-Driven Development of Ontologies",
booktitle="The Semantic Web. Latest Advances and New Domains",
year="2016",
publisher="Springer International Publishing",
address1 = "Cham, Switzerland",
pages="642--657",
doi1={10.1007/978-3-319-34129-3_39}
}

@article{KeetDataset2020,
title = {Dataset of ontology competency questions to SPARQL-OWL queries translations},
journal = {Data in Brief},
volume = {29},
pages = {105098},
year = {2020},
issn1 = {2352-3409},
doi1 = {10.1016/j.dib.2019.105098},
author = {Jedrzej Potoniec and Dawid Wiśniewski and Agnieszka Ławrynowicz and C. Maria Keet}
}


@inproceedings{Bezerra2017duplicatetoremove,
  author       = {Camila Bezerra and
                  Fred Freitas},
  editor1       = {Mara Abel and
                  Sandro Rama Fiorini and
                  Christiano Pessanha},
  title        = {Verifying Description Logic Ontologies based on Competency Questions
                  and Unit Testing},
  booktitle1    = {Proceedings of the {IX} Seminar on Ontology Research in Brazil and
                  {I} Doctoral and Masters Consortium on Ontologies, Bras{\'{\i}}lia,
                  Brazil, August 28th-30th, 2017},
booktitle    = {Proceedings of the {IX} Seminar on Ontology Research in Brazil and
                  {I} Doctoral and Masters Consortium on Ontologies},
  series       = {{CEUR} Workshop Proceedings},
  volume       = {1908},
  pages        = {159--164},
  publisher    = {CEUR-WS.org},
  year         = {2017}
}

@article{Deng_Lin_2023, 
title={The Benefits and Challenges of ChatGPT: An Overview},
volume={2}, 
DOI1={10.54097/fcis.v2i2.4465}, 
number={2}, 
journal={Frontiers in Computing and Intelligent Systems}, 
author={Deng, Jianyang and Lin, Yijia}, 
year={2023}, 
pages={81–83} }

@ARTICLE{Dave2023,
  title    = "{ChatGPT} in medicine: an overview of its applications,
              advantages, limitations, future prospects, and ethical
              considerations",
  author   = "Dave, Tirth and Athaluri, Sai Anirudh and Singh, Satyam",
  journal  = "Front Artif Intell",
  volume   =  "6",
  pages    = "1169595",
  year     =  "2023",
  
}

@INPROCEEDINGS{Qadir2023,
  author={Qadir, Junaid},
  booktitle={2023 IEEE Global Engineering Education Conference (EDUCON)}, 
  title={Engineering Education in the Era of ChatGPT: Promise and Pitfalls of Generative AI for Education}, 
  year={2023},
  volume={},
  number={},
  pages={1-9},
  doi1={10.1109/EDUCON54358.2023.10125121}}

@inproceedings{reimers-gurevych-2019-sentence,
    title = "Sentence-{BERT}: Sentence Embeddings using {S}iamese {BERT}-Networks",
    author = "Reimers, Nils  and
      Gurevych, Iryna",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    year = "2019",
    publisher = "Association for Computational Linguistics",
    doi1 = "10.18653/v1/D19-1410",
    pages = "3982--3992"   
}

@article{Parkkila2017AnOF,
  title={An ontology for videogame interoperability},
  author={Janne Parkkila and Filip Radulovic and Daniel Garijo and Mar{\'i}a Poveda-Villal{\'o}n and Jouni Ikonen and Jari Porras and Asunci{\'o}n G{\'o}mez-P{\'e}rez},
  journal={Multimedia Tools and Applications},
  year={2017},
  volume={76},
  pages={4981-5000}
}

@techreport{smartm2m,
    title = {SmartM2M: SAREF Extension Investigation},
    type = {Technical Report},
    number = {TR 103 411},
    year={2017}
}

@book{montiel2011multilingualism,
  title={Multilingualism in Ontologies - Building Patterns and Representation Models},
  author={Montiel-Ponsoda, E.},
  publisher={LAP Lambert Academic Publishing},
  address1={Germany},
  year={2011}
}

@InProceedings{Aziz2023,
author="Azzi, Sabrina
and Assi, Ali
and Gagnon, St{\'e}phane",
editor1="Garoufallou, Emmanouel
and Vlachidis, Andreas",
title="Scoring Ontologies for Reuse: An Approach for Fitting Semantic Requirements",
booktitle="Metadata and Semantic Research",
year="2023",
publisher="Springer Nature",
address1 = "Cham, Switzerland",
pages="203--208",
doi1={10.1007/978-3-031-39141-5_17}
}

@inproceedings{alharbiKcap2021,
author = {Alharbi, Reham and Tamma, Valentina and Grasso, Floriana},
title = {Characterising the Gap Between Theory and Practice of Ontology Reuse},
year = {2021},
publisher = {ACM},
booktitle = {Proceedings of the 11th on Knowledge Capture Conference},
pages = {217–224},
numpages = {8},
series = {K-CAP '21}
}

@article{GangemiEtAl2017,
  author = {Gangemi, Aldo and Presutti, Valentina and Recupero, Diego Reforgiato and Nuzzolese, Andrea Giovanni and Draicchio, Francesco and MongiovÃ¬, Misael},
  journal = {Semantic Web},
  number = 6,
  pages = {873-893},
  title = {{Semantic Web Machine Reading with FRED}},
  volume = 8,
  year = 2017
}

@inproceedings{DBLP:conf/acl/ImaniD023,
  author       = {Shima Imani and
                  Liang Du and
                  Harsh Shrivastava},
  title        = {MathPrompter: Mathematical Reasoning using Large Language Models},
  booktitle1    = {Proceedings of the The 61st Annual Meeting of the Association for
                  Computational Linguistics: Industry Track, {ACL} 2023, Toronto, Canada,
                  July 9-14, 2023},
 booktitle1    = {Proceedings of the The 61st Annual Meeting of the Association for
                  Computational Linguistics: Industry Track, {ACL} 2023},
  pages        = {37--42},
  year         = {2023},
}

@inproceedings{AlkhuzaeyECEL23,
  title={A Framework for Assessing the Complexity of Auto Generated Questions from Ontologies},
  author={Samah AlKhuzaey and Floriana Grasso and Terry R. Payne and Valentina Tamma},
  booktitle={Proc. of the 22nd European Conf. on e-Learning (to appear)},
  year={2023}
}

@book{10.1145/3382097, 
author = {Allemang, Dean and Hendler, Jim and Gandon, Fabien}, title = {Semantic Web for the Working Ontologist: Effective Modeling for Linked Data, RDFS, and OWL}, year = {2020}, isbn = {9781450376174}, publisher = {Association for Computing Machinery}, address1 = {New York, NY, USA}, edition = {3}, volume = {33}, abstract = {Enterprises have made amazing advances by taking advantage of data about their business to provide predictions and understanding of their customers, markets, and products. But as the world of business becomes more interconnected and global, enterprise data is no long a monolith; it is just a part of a vast web of data. Managing data on a world-wide scale is a key capability for any business today.The Semantic Web treats data as a distributed resource on the scale of the World Wide Web, and incorporates features to address the challenges of massive data distribution as part of its basic design. The aim of the first two editions was to motivate the Semantic Web technology stack from end-to-end; to describe not only what the Semantic Web standards are and how they work, but also what their goals are and why they were designed as they are. It tells a coherent story from beginning to end of how the standards work to manage a world-wide distributed web of knowledge in a meaningful way.The third edition builds on this foundation to bring Semantic Web practice to enterprise. Fabien Gandon joins Dean Allemang and Jim Hendler, bringing with him years of experience in global linked data, to open up the story to a modern view of global linked data. While the overall story is the same, the examples have been brought up to date and applied in a modern setting, where enterprise and global data come together as a living, linked network of data. Also included with the third edition, all of the data sets and queries are available online for study and experimentation at data.world/swwo.} }


%%%%% THE END OF KCAP 2023 BIB %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%% THE END OF KCAP 2023 BIB %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

